Enabling Conversational Behavior Reasoning Capabilities in Full-Duplex Speech

Human conversation is organized by an implicit chain of thoughts that manifests as timed speech acts. Capturing this causal pathway is key to building natural full-duplex interactive systems. We introduce a framework that enables reasoning over conversational behaviors by modeling this process as causal inference within a Graph-of-Thoughts (GoT). Our approach formalizes the intent-to-action pathway with a hierarchical labeling scheme, predicting high-level communicative intents and low-level speech acts to learn their causal and temporal dependencies. To train this system, we develop a hybrid corpus that pairs controllable, event-rich simulations with human-annotated rationales and real conversational speech. The GoT framework structures streaming predictions as an evolving graph, enabling a multimodal transformer to forecast the next speech act, generate concise justifications for its decisions, and dynamically refine its reasoning. Experiments on both synthetic and real duplex dialogues show that the framework delivers robust behavior detection, produces interpretable reasoning chains, and establishes a foundation for benchmarking conversational reasoning in full duplex spoken dialogue systems.

==> dataset.tex <==
\subsection{Dataset}
\label{sec:dataset}

We use both synthetic (simulation) and real conversational audio for training and evaluation. All datasets are partitioned into train/validation/test splits in an 8:1:1 ratio.

For the synthetic simulation corpus, narrative prompts are taken from the \textsc{ExploreToM} dataset and used as input to an LLM-based text generation stage. Dialogue text is generated from each narrative using \texttt{gpt-4o-mini}; the same model is prompted to mark candidate backchannel and interruption points which are used to place event labels. Speech waveforms are synthesized from the generated dialogue text with \texttt{CosyVoice2}. To increase stability and consistency of synthesized voice quality across clips, the synthesizer is conditioned on a timbre reference audio clip drawn from an external dataset (the specific external dataset will be specified in a later version). For backchannel and interruption cases we synthesize controlled overlap between the two speakers so that samples include partial overlap.

The simulation corpus contains approximately \textbf{28,000} synthesized audio clips totaling roughly \textbf{192 hours}. To support Graph-of-Thought (GoT) supervision, we generate second-level rationale annotations for the simulation audio using the OpenAI API: for each second \(t\) the model is prompted with only the text up to \(t\) and asked to produce a rationale for that second. Because the automatic outputs include errors, generated rationales were manually validated and corrected; the resulting GoT annotation set contains approximately \textbf{37,100} second-level rationale entries.

Event counts in the simulation corpus (turn-taking : interruption : backchannel : continuation) were provided as \(97:149:54:548\), corresponding to approximately \textbf{11.4\%}, \textbf{17.6\%}, \textbf{6.4\%}, and \textbf{64.6\%} respectively. Compared to the Talking-Turns benchmark \citep{arxiv:2503.01174}, which reports lower proportions of interruptions and backchannels in human dialogue (≈0.4\% each in-domain), our synthetic corpus deliberately upweights these events to provide stronger supervision signals for detection and modeling.

For real (non-synthetic) data we use the CANDOR conversational corpus. The full resource is a large-scale dataset of recorded natural conversations; for our experiments we select a curated subset totaling \textbf{118 hours} of audio.


==> related_study.tex <==
\section{Related Study}
\label{sec:related}

Conversational turn-taking and speech-event modeling are central topics in spoken dialogue research. Early operationalizations of talking turns and chunk-wise turn events have been used to define low-level labels (e.g., continuation, turn-change, backchannel), which many subsequent works adopt for annotation and evaluation \citep{arxiv:2503.01174}. Building on these definitions, we follow the same fine-grained segmentation for our low-level speech-act labels.

At a higher level, speech-act and intent taxonomies from classical pragmatics and computational pragmatics motivate structured high-level categories (inform, request, assess, etc.), which are useful for mapping event detections to discourse intent. These taxonomies inform the high-level labels we employ and how they compose with low-level events.

A number of modeling approaches address automatic detection of speech events. Voice Activity Projection (VAP) has been proposed as a self-supervised objective to predict future voice activity and has been adapted for frame-wise backchannel and turn-taking prediction \citep{arxiv:2410.15929,arxiv:2503.01174}. Complementary approaches fuse acoustic encoders with large language models to leverage both prosodic cues and linguistic priors for more accurate turn-taking and backchannel localization \citep{arxiv:2401.14717}. To support evaluation and training, recent benchmarks and datasets target full-duplex phenomena (pauses, overlaps, interruptions, backchannels); for example, Full-Duplex-Bench provides systematic metrics and scenarios for assessing pause handling, backchannel timing, turn-taking, and interruption management \citep{arxiv:2503.04721}, while Behavior-SD supplies a large synthetic spoken-dialogue corpus with speaker-level behavioral annotations and a behavior-conditioned generation model \citep{behavior-sd}. Generative, textless spoken-dialogue models such as dGSLM demonstrate that multi-channel, textless modeling can reproduce paralinguistic signals and more naturalistic turn dynamics, which is relevant for behavior-conditioned generation and simulation \citep{arxiv:2203.16502}.

Taken together, these prior studies motivate our hierarchical design: (i) adopt established low-level event definitions from turn-taking benchmarks, (ii) incorporate high-level intent taxonomies for pragmatic labeling, (iii) use behavior-conditioned simulation datasets for targeted augmentation, and (iv) supervise a graph-based inference component to recover rationale among events, content, and intents.

